Segment Everything Everywhere All at Once

In this work, we present SEEM, a promptable and interactive model for segmenting everything everywhere all at once in an image, as shown in Fig.1. In SEEM, we propose a novel decoding mechanism that enables diverse prompting for all types of segmentation tasks, aiming at a universal segmentation interface that behaves like large language models (LLMs). More specifically, SEEM is designed with four desiderata: i) Versatility. We introduce a new visual prompt to unify different spatial queries including points, boxes, scribbles and masks, which can further generalize to a different referring image; ii) Compositionality. We learn a joint visual-semantic space between text and visual prompts, which facilitates the dynamic composition of two prompt types required for various segmentation tasks; iii) Interactivity. We further incorporate learnable memory prompts into the decoder to retain segmentation history through mask-guided cross-attention from decoder to image features; and iv) Semantic-awareness. We use a text encoder to encode text queries and mask labels into the same semantic space for open-vocabulary segmentation. We conduct a comprehensive empirical study to validate the effectiveness of SEEM across diverse segmentation tasks. Notably, our single SEEM model achieves competitive performance across interactive segmentation, generic segmentation, referring segmentation, and video object segmentation on 9 datasets with minimum 1/100 supervision. Furthermore, SEEM showcases a remarkable capacity for generalization to novel prompts or their combinations, rendering it a readily universal image segmentation interface.

==> sec/imgs/compare.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{sec/imgs/concept_xyz.png}
    \vspace{-2pt}
    \caption{Comparison with concurrent work SAM~\cite{kirillov2023segment}. Our approach has richer context on both interaction approaches (e.g. Referring region of an example image) as well as semantic spaces (support class aware segmentation).
    % The x-axis and y-axis denote the level of interaction and semantics. 
    % We compare the levels of interaction and semantics of three segmentation tasks (edge detection, open-set, and interactive segmentation). Open-set Segmentation usually requires a high level of semantics and does not require interaction. Compared with SAM, \ourmodel{} covers a larger range in both interaction and semantics levels, as it supports more prompt types and understands semantics (summarized in Fig.~\ref{fig:teaser}). 
    % For example, SAM only supports limited interaction types like points and boxes, and it does not support high-semantic tasks since it does not output semantic labels itself. 
    % Note that although we do not report edge detection results, our model can support it by simply converting masks to edges.
    }
    % is trained on a large amount of segmentation data to do interactive segmentation. Though SAM advances the progress of vision understanding, however, it can not predict semantic labels. In addition, it only supports a limited number of interaction types like points and boxes. \ourmodel{} attempts to move one step forward to these two challenging problems and learn a universal segmentation model.}
    \vspace{-.4cm}
    \label{fig:compare}
\end{figure}
